Better Algorithms for Constructing Minimum Cost Markov Chains and AIFV Codes

The problem of constructing optimal AIFV codes is a special case of that of constructing minimum cost Markov Chains. This paper provides the first complete proof of correctness for the previously known iterative algorithm for constructing such Markov chains. A recent work describes how to efficiently solve the Markov Chain problem by first constructing a Markov Chain Polytope and then running the Ellipsoid algorithm for linear programming on it. This paper's second result is that, in the AIFV case, a special property of the polytope instead permits solving the corresponding linear program using simple binary search

==> MainTheorem.tex <==
\begin{theorem} \label{thm : 1}
    There exists a unique multi-colored intersection point on $H$.
\end{theorem}

\begin{proof}
    First, we prove the existence of such a point. Note that the multi-colored intersection points of hyperplanes are finite because the set of hyperplanes of each type is assumed to be finite.

    Assume $\vecp_0 \in \R^{m-1}$ is the projection of an arbitrary multi-colored intersection point on $\R^{m-1}$ subspace of $\R^m$, i.e. if the corresponding hyperplanes are $f_i \lp \x,S_i \rp $, we have
    \[
        \forall i,j \in  \la 0,1,\dots,m-1 \ra  : f_i \lp \vecp_0 ,S_i \rp  = f_j \lp \vecp_0,S_j \rp 
    \]
    We construct the sequence $ \la \vecp_i \ra _{i \in \N \cup  \la  0 \ra }$ of elements of $\R^{m-1}$ as follows:

    For each $i \in \N$, $\vecp_i$ is the projection of the intersection point of the hyperplanes defined by the following trees:

    \begin{equation}
        \S_{i-1} =  \T \lp \vecp_{i-1} \rp
    \end{equation}

    Note that since the hyperplanes are finite, the set $ \la \vecp_0, \vecp_1, \dots  \ra $ is finite too.

    According to the definition of the sequence, we can define the sequence $ \la c_i \ra _{i \in \N \cup  \la  0 \ra }$  ( which is the sequences of costs of corresponding Markov chains of intersection points in the sequence $ \la \vecp_i \ra _{i \in \N \cup  \la  0 \ra }$  )   as below:

    \begin{equation} \label{eq : def of costs}
        c_i = f_1 \lp \vecp_i,S_0 \lp \vecp_{i-1} \rp  \rp  = f_1 \lp \vecp_i,S_1 \lp \vecp_{i-1} \rp  \rp  = \dots = f_{m-1} \lp \vecp_i,S_{m-1} \lp \vecp_{i-1} \rp  \rp 
    \end{equation}

    \begin{claim} \label{clm: convergence of costs}
        For all $i \in \N$, $c_i \leq c_{i-1}$ and if equality holds, we have $\vecp_i \leq \vecp_{i-1}$.
    \end{claim}
    \begin{proof}
        We know $c_{i-1} \geq f_j \lp \vecp_{i-1},S_j \lp \vecp_{i-1} \rp  \rp $ for all $j$ because of \ref{eq : def of costs}. According to lemma \ref{lem : main lemma}, there exists an index $j > 0$ s.t.

        \[
            f_j \lp \vecp_{i-1},S_j \lp \vecp_{i-1} \rp  \rp  > f_j \lp \vecp_i,S_j \lp \vecp_{i-1} \rp  \rp  = c_i
        \]
        or if $\vecp_i \leq \vecp_{i-1}$,
        \[
            f_0 \lp \vecp_{i-1},S_0 \lp \vecp_{i-1} \rp  \rp  \geq f_0 \lp \vecp_i,S_0 \lp \vecp_{i-1} \rp  \rp  = c_i
        \]
        and the claim is proved.
    \end{proof}
    As a result of the claim above, and the fact that the intersection points are finite, we can conclude that the sequence $ \la c_i \ra _{i \in \N \cup  \la  0 \ra }$ converges.

    Here is the main claim which allows us to conclude the statement of the theorem.

    \begin{claim} \label{clm: main claim}
        There exists $N \in \N$ s.t. for all $i > N$ we have $\vecp_i \geq \vecp_{i+1}$; moreover, by finiteness of the set $ \la \vecp_0, \vecp_1, \dots  \ra $, for all sufficiently large $n \in \N$, $\vecp_n = \vecp_{n+1}$.
    \end{claim}

    Pay attention that if $\vecp_n = \vecp_{n+1}$ for sufficiently large $n$ s.t. $c_n = c_{n+1}$, it means the hyperplanes passing through the points $[\vecp_n ,c_n]^T$ and $[\vecp_{n+1},c_{n+1}]^T$ are the same; therefore, $[\vecp_n,c_n]^T$ lies on the intersection of all $m$ lower-envelopes, i.e.
    \[
        \forall k: c_n = g_k \lp \vecp_n \rp 
    \]
    hence,
    \[
        c_n = h \lp \vecp_n \rp 
    \]
    and therefore, $[\vecp_n,c_n]^T$ is a multi-colored intersection point on $H$ and the first part of the theorem will be proved.
    
    \begin{proof}
        Assume for the contrary that $\vecp_i \leq \vecp_{i-1}$ does not hold for infinitely many $i \in \N$. By claim \ref{clm: convergence of costs} we know $c_i < c_{i-1}$; therefore, the sequence $ \la c_i \ra $ strictly decreases infinitely many times, hence, the set $ \la c_0,c_1,\dots \ra $ is infinite which is a contradiction; because the set of intersection points is finite.
    \end{proof}
    And the existence part is completed.

    To prove the uniqueness, assume $Q = [\x ,h]^T$ and $Q'=[\x',h]^T$  ( $Q,Q' \in \R^m$ and $\x \in \R^{m-1}$ )   are multi-colored points on the top of the $H$. It is sufficient to show that $Q = Q'$. Assume $Q \leq Q'$ doesn't hold. Therefore, by lemma \ref{lem : main lemma}, there exists an index $i$ s.t.
    
    \begin{equation}\label{eq: uniqueness ineq}
        f_i \lp \x,S_i \rp  > f_i \lp \x',S_i \rp  
    \end{equation}

    for all $S_i$. Thus, if $f_i \lp \x,S_i \rp $ passes through $Q$, the following inequality contradict our assumption:
    \[
        f_i \lp \x,S_i \rp  = h = h \lp \x' \rp  \leq f_i \lp \x',S_i \rp 
    \]
    which is a contradiction since  ( \ref{eq: uniqueness ineq}  )   holds. Hence
    \[
        Q \leq Q'
    \]
    Similarly, we can conclude $Q' \leq Q$ and thus, $Q = Q'$ and we are done.
\end{proof}
